Robust Approximate Simulation for Hierarchical Control of Piecewise Affine Systems under Bounded Disturbances

Piecewise affine (PWA) systems are widely applied in many practical cases such as the control of nonlinear systems and hybrid dynamics. However, most of the existing PWA control methods have poor scalability with respect to the number of modes and system dimensions and may not be robust to the disturbances in performance. In this paper, we present a robust approximate simulation based control method for PWA systems under bounded external disturbances. First, a lower-dimensional linear system (abstraction) and an associated interface are designed to enable the output of the PWA system (concrete system) to track the output of the abstraction. Then, a Lyapunov-like simulation function is designed to show the boundedness of the output errors between the two systems. Furthermore, the results obtained for linear abstraction are extended to the case that a simpler PWA system is the abstraction. To illustrate the effectiveness of the proposed approach, simulation results are provided for two design examples.

==> additional.tex <==
To determine the corresponding partition in the abstraction's space, i.e. \(\mathbf{D}_{zj}z\geq \mathbf{E}_{zj}\), based on the desired partition in concrete system's space, i.e. \(\mathbf{D}_{j}x\geq \mathbf{E}_{j}\), the following lemma is applied:

\begin{lemma} \cite{??,??}
    Given a polytope \(\mathcal{Z}=\{\mathbf{z}\in\mathbb{R}^m|\mathbf{D}_{zj}\mathbf{z}\geq \mathbf{E}_{zj}\}\), \(\mathbf{P}_i\in\mathbb{R}^{n\times m}\), \(\mathbf{\hat{y}}\in\mathbb{R}^n\), and \(\mathcal{X}_j=\{\mathbf{x}\in\mathbb{R}^n|\mathbf{D}_j\mathbf{x}\geq \mathbf{E}_j\}\), \(j=1,...,r\), the condition \(\mathbf{P}_i\mathcal{Z}+\mathbf{\hat{y}}\subseteq\mathcal{X}_j\) is equivalent to
    \begin{equation}
        \mathbf{\Lambda}_k\mathbf{D}_{zj}=\mathbf{D}_{j}\mathbf{Q}_k,\ \sum_{k=1}^{N}\mathbf{\Lambda}_k\mathbf{E}_{zj}\geq \mathbf{E}_j-\mathbf{D}_{j}\mathbf{\hat{y}}
    \end{equation}
    where \(\mathbf{\Lambda}_k\) is some matrix with nonnegative entries, \(\sum_{k=1}^{N} \mathbf{Q}_k=\mathbf{P}_i\).
\end{lemma}
